Evaluating the Information Security Awareness of Smartphone Users

Information security awareness (ISA) is a practice focused on the set of skills, which help a user successfully mitigate a social engineering attack. Previous studies have presented various methods for evaluating the ISA of both PC and mobile users. These methods rely primarily on subjective data sources such as interviews, surveys, and questionnaires that are influenced by human interpretation and sincerity. Furthermore, previous methods for evaluating ISA did not address the differences between classes of social engineering attacks. In this paper, we present a novel framework designed for evaluating the ISA of smartphone users to specific social engineering attack classes. In addition to questionnaires, the proposed framework utilizes objective data sources: a mobile agent and a network traffic monitor; both of which are used to analyze the actual behavior of users. We empirically evaluated the ISA scores assessed from the three data sources (namely, the questionnaires, mobile agent, and network traffic monitor) by conducting a long-term user study involving 162 smartphone users. All participants were exposed to four different security challenges that resemble real-life social engineering attacks. These challenges were used to assess the ability of the proposed framework to derive a relevant ISA score. The results of our experiment show that: (1) the self-reported behavior of the users differs significantly from their actual behavior; and (2) ISA scores derived from data collected by the mobile agent or the network traffic monitor are highly correlated with the users' success in mitigating social engineering attacks.

==> Resources/comparison_table.tex <==
{
\begin{table}[H]

\begin{footnotesize}
\begin{tabularx}{\textwidth}{| >{\bf}Y | Y | Y | Y |}

\hline
&   \textbf{Questionnaire}
&   \textbf{Network-based analysis}
&   \textbf{Mobile agent} \\

\hline
    Level of interaction with the subject      
&   Very high
&   Medium
&	None \\

\hline
Level of invasiveness
&   Low
&   High &	Medium \\

\hline
Required tracking time
& Low
& Medium
& High  \\

\hline
Objectivity level of the analysis 
& Low
& High
& High  \\

\hline

\end{tabularx}
\end{footnotesize}
\caption{A comparison between the three data sources}\label{tab:comparison}
\end{table}

}

==> Resources/taxonomy_table_2.tex <==
{

\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\begin{scriptsize}

\begin{longtable}{| M{\textwidth*3/16} | M{\textwidth/18} | p{\textwidth*11/16} |}

%>{\raggedright}
\hline
\textbf{Topics} & \textbf{ID} & \textbf{Behavior} \\ 
\hline
\multicolumn{3}{|c|}{\textbf{Focus area:} Applications \textbf{Sub-Focus area:} Application Installation (AI)}\\
\hline
\multirow{2}{\hsize}{\centering Untrusted Sources}
 				& \multirow{2}{\hsize}{\centering AI1}  & Validates the source of applications before installation. Installs applications solely from trusted sources.\\\cline{3-3}
                &  					& Installs applications solely from trusted sources.\\
 				
	\hline
\multirow{2}{\hsize}{\centering Permissions}
 				& \multirow{2}{\hsize}{\centering AI2}  & Does not install applications that require dangerous permissions.\\\cline{3-3}
                &  						& Manages the permissions granted to applications properly.\\
 				
	\hline
\multirow{2}{\hsize}{\centering Rating}
 				& \multirow{2}{\hsize}{\centering AI3}  & Validates the rating of an application.\\\cline{3-3}
                &  						& Does not install applications with a low rating.\\
 				
	\hline   
\multirow{2}{\hsize}{\centering Root/Jailbreak} 
 				& \multirow{2}{\hsize}{\centering AI4}  & Rarely installs applications that require root privileges.\\\cline{3-3}
                &  						& Manages root privileges properly.\\
 				
	\hline      
\multirow{2}{\hsize}{\centering Unknown/ Unsigned Applications} 
 				& \multirow{2}{\hsize}{\centering AI5}  & Configures the OS to prevent the installation of unsigned applications on the device and does not download or install unknown/ unsigned applications.\\\cline{3-3}
                &  						& Operates the OS in accordance with system alerts.\\
 				
	\hline
\multicolumn{3}{|c|}{\textbf{Focus area:} Applications \textbf{Sub-Focus area:} Application Handling (AH)}\\
\hline
\multirow{2}{\hsize}{\centering Security Updates} 
 				& \multirow{2}{\hsize}{\centering AH1}  & Configures the OS to update applications automatically.\\\cline{3-3}
                &  						& Does not postpone security updates.\\
 				
	\hline 
\multirow{2}{\hsize}{\centering Malicious Updates}
 				& \multirow{2}{\hsize}{\centering AH2}  & Does not allow automatic updates of untrusted applications.\\\cline{3-3}
                &  						& Does not perform updates that require sensitive permissions and removes irrelevant/unused/dangerous applications from the device.\\
 				
	\hline 
\multirow{2}{\hsize}{\centering Permissions} 
 				& \multirow{2}{\hsize}{\centering AH3}  & Does not install applications that require sensitive permissions.\\\cline{3-3}
                &  						& Manages application permissions properly and restricts applications’ access to sensitive and unrelated resources.\\
 				
	\hline 

\multirow{2}{\hsize}{\centering Application Advertisements} 
 				& \multirow{2}{\hsize}{\centering AH4}  & Rarely clicks on advertisements.\\\cline{3-3}
                &  						& Does not insert private information into advertiser's websites before validating it. \\
 				
	\hline     
    
\multirow{2}{\hsize}{\centering Privacy Settings} 
 				& \multirow{2}{\hsize}{\centering AH5}  & Properly configures applications' privacy settings to preserve privacy.\\\cline{3-3}
                &  						& Operates in accordance with security alerts.\\
 				
	\hline     
        
\multicolumn{3}{|c|}{\textbf{Focus area:} Browsing and Communications  \textbf{Sub-Focus area:} Browser (B)}\\\hline    
    
\multirow{2}{\hsize}{\centering Malicious Sites} 
 				& \multirow{2}{\hsize}{\centering B1}  & Validates suspicious domains and does not enter malicious domains.\\\cline{3-3}
                &  						& Operates in accordance with security alerts.\\
 				
	\hline    
\multirow{2}{\hsize}{\centering Certificates - General} 
 				& \multirow{2}{\hsize}{\centering B2}  & Prefers to use HTTPS sites.\\\cline{3-3}
                &  						& Does not operate via HTTP in domains that support HTTPS.\\
 				
	\hline       
\multirow{2}{\hsize}{\centering Certificates – File Downloads} 
 				& \multirow{2}{\hsize}{\centering B3}  & Prefers to download files via HTTPS.\\\cline{3-3}
                &  						& Validates the file’s checksum if the file has been downloaded via HTTP.\\
 				
	\hline    

\multirow{2}{\hsize}{\centering Certificates – Data Confidentiality} 
 				& \multirow{2}{\hsize}{\centering B4}  & Prefers to use HTTPS sites.\\\cline{3-3}
                &  						& Does not send sensitive information via HTTP.\\
 				
	\hline 
\multirow{2}{\hsize}{\centering Pop-up Blockers} 
 				& \multirow{2}{\hsize}{\centering B5}  & Uses pop-up blockers.\\\cline{3-3}
                &  						& Does not insert private information into pop-ups.\\
 				
	\hline    
\multirow{2}{\hsize}{\centering Certificates – Deletion } 
 				& \multirow{2}{\hsize}{\centering B6}  &  Deletes unknown certificates from the device.\\\cline{3-3}
                &  						& Operates in accordance with system/browser alerts and does not use untrusted certificates.\\
 				
	\hline     
\multirow{2}{\hsize}{\centering Advertisements/ Advertising Sites} 
 				& \multirow{2}{\hsize}{\centering B7}  &  Uses advertisement blockers.\\\cline{3-3}
                &  						& Does not insert private information on advertisers' sites.\\
 				
	\hline     
\multirow{2}{\hsize}{\centering Certificates – Installation} 
 				& \multirow{2}{\hsize}{\centering B8}  &   Carefully manages the certificates on the device.\\\cline{3-3}
                &  						& Operates in accordance with system/browser alerts and does not install untrusted certificates.\\		
	\hline   
\multirow{2}{\hsize}{\centering Certificates – Validation} 
 				& \multirow{2}{\hsize}{\centering B9}  &  Does not operate with untrusted certificates.\\\cline{3-3}
                &  						& Validates domain certificates and operates in accordance with system/browser alerts.\\		
	\hline  
\multirow{2}{\hsize}{\centering Plugins, Add-ons, Extensions} 
 				& \multirow{2}{\hsize}{\centering B10}  &  Properly manages the plugins/add-ons/extensions installed on his/her browser and erases unwanted plugins.\\\cline{3-3}
                &  						& Validates the signature and source of a plugin before installation.\\		
	\hline  
Private Browsing & B11  & Rarely inserts private data on a device that is not owned by the user (or on a shared device).\\
	\hline  

\multicolumn{3}{|c|}{\textbf{Focus area:} Browsing and Communications  \textbf{Sub-Focus area:} Virtual Communication (VC)}\\\hline    

\multirow{2}{\hsize}{\centering Malicious Hyperlinks} 
 				& \multirow{2}{\hsize}{\centering VC1}  & Does not click on suspicious hyperlinks.\\\cline{3-3}
                &  						& Uses incognito mode (i.e., private browsing) while using a device that is not owned by the user (or a share device).\\		
	\hline  
\multirow{2}{\hsize}{\centering Unknown Sender (Spammer)} 
 				& \multirow{2}{\hsize}{\centering VC2}  & Validates the sender of an email.\\\cline{3-3}
                &  						& Does not open emails/messages received from unknown senders (or spam).\\		
	\hline  
Unknown Sender/Spam – Hyperlinks & VC3  & Validates URLs embedded in emails.\\
	\hline  
    
\multirow{2}{\hsize}{\centering Unknown Sender – Malicious Attachments}
 				& \multirow{2}{\hsize}{\centering VC4}  &  Validates attachments received from unknown senders (or spammers).\\\cline{3-3}
                &  						& Does not download and/or execute file attachments classified as malicious or received from unknown senders.\\		
	\hline  
    
\multirow{2}{\hsize}{\centering Advertisements} 
 				& \multirow{2}{\hsize}{\centering VC5}  &  Validates the sender.\\\cline{3-3}
                &  						& Does not open advertisement emails received form unknown senders.\\		
	\hline  
    
\multirow{2}{\hsize}{\centering Junk Mailbox} 
 				& \multirow{2}{\hsize}{\centering VC6}  &  Validates the sender of an email. \\\cline{3-3}
                &  						&  Does not open/read messages/emails classified as spam.\\		
	\hline     
  
\multicolumn{3}{|c|}{\textbf{Focus area:} Device  \textbf{Sub-Focus area:} Operating Systems (OS)}\\\hline    

\multirow{2}{\hsize}{\centering Updates} 
 				& \multirow{2}{\hsize}{\centering OS1}  &  Uses an updated OS and configures auto-updates for critical services. \\\cline{3-3}
                &  						&  Does not postpone critical updates of the OS (e.g., by ignoring update alerts).\\
	\hline 
Vulnerable OS & OS2  & Does not use an OS with known vulnerabilities and stays updated regarding known vulnerabilities of his/her OS. \\
	\hline     
\multirow{2}{\hsize}{\centering Root/Jailbreak} 
 				& \multirow{2}{\hsize}{\centering OS3}  &   Does not root or jailbreak the device. \\\cline{3-3}
                &  						&  Properly manages super-user privileges (in case he/she must root the device).\\
	\hline
\multicolumn{3}{|c|}{\textbf{Focus area:} Device \textbf{Sub-Focus area:} Data Privacy (DP)}\\\hline    
\multirow{2}{\hsize}{\centering Encryption} 
 				& \multirow{2}{\hsize}{\centering DP1}  &  Encrypts the drive of the device.\\\cline{3-3}
                &  						&  Does not share his/her PIN-code with others.\\
    \hline
Backup & DP2 &  Uses backup services.\\
    \hline    
Private Data & DP3 & Does not store sensitive material on the device.\\
	\hline
\multicolumn{3}{|c|}{\textbf{Focus area:} Device \textbf{Sub-Focus area:} Security Systems (SS)}\\
	\hline   
\multirow{2}{\hsize}{\centering Embedded Security Systems}
 				& \multirow{2}{\hsize}{\centering SS1}  & Uses embedded security systems.\\\cline{3-3}
                &  						& Does not ignore security alerts related to the embedded security systems.\\
    \hline
\multirow{2}{\hsize}{\centering Antivirus} 
 				& \multirow{2}{\hsize}{\centering SS2}  & Uses antivirus application regularly to scan the device.\\\cline{3-3}
                &  						& Does not ignore security alerts from the antivirus application.\\
    \hline
    
\multirow{2}{\hsize}{\centering Mobile Device Management} & \multirow{2}{\hsize}{\centering SS3}  & Uses MDM services.\\\cline{3-3}
                 &  						& Does not ignore security alerts from the MDM application.\\
    \hline
Security Updates & SS4 & Updates security systems.\\
    \hline
Security Alerts  & SS5 & Operates in accordance with security alerts (i.e., does not ignore security alerts).\\
    \hline
\multirow{2}{\hsize}{\centering Remote Deletion Services} & \multirow{2}{\hsize}{\centering SS6}  & Installs remote deletion services on the device.\\\cline{3-3}
                 &  						& Erases the device if it has been lost.\\
    \hline
\multirow{2}{\hsize}{\centering PIN-code} & \multirow{2}{\hsize}{\centering SS7}  & Uses PIN-codes/patterns/ fingerprinting.\\\cline{3-3}
                 &  						& Does not share his/her PIN-code with others.\\
    \hline
    
\multicolumn{3}{|c|}{\textbf{Focus area:} Communication Channels \textbf{Sub-Focus area:} Networks (N)}\\
	\hline
Wi-Fi – Auto-Connect & N1  &  Does not auto-connect to unknown Wi-Fi networks.\\
    \hline
Wi-Fi – Unencrypted Networks & N2  & Does not connect to unencrypted networks.\\
    \hline   
\multirow{2}{\hsize}{\centering Wi-Fi – Unencrypted Networks} & \multirow{2}{\hsize}{\centering N3}  & Does not download files on unencrypted Wi-Fi networks.\\\cline{3-3}
                 &  						& Validates the signature of files and does not execute a file with an incorrect signature.\\
    \hline
VPN   & N4  &  Uses VPN services on public networks.\\  
    \hline
Wi-Fi – Unencrypted Networks & N5 & Does not transmit private data via unencrypted channels.\\
	\hline
\multicolumn{3}{|c|}{\textbf{Focus area:} Communication Channels \textbf{Sub-Focus area:} Physical Channels (PC)}\\
	\hline
NFC/Bluetooth & PC1 & Enables Bluetooth and NFC while they are in use and only connects trusted Bluetooth and NFC devices.\\
	\hline
USB/Charging Connections & PC2 &  Does not use a USB to connect the device to unknown devices.\\
	\hline
\multirow{2}{\hsize}{\centering Physical Access} & \multirow{2}{\hsize}{\centering PC3}  & Does not keep the device unattended and uses a PIN-code.\\\cline{3-3}
                 &  						&  Does not share his/her PIN-code with others.\\
    \hline
\end{longtable}
\end{scriptsize}


}
